Searching for new physics at $\mu\rightarrow e$ facilities with $\mu^+$ and $\pi^+$ decays at rest

We investigate the ability of $\mu\rightarrow e$ facilities, Mu2e and COMET, to probe, or discover, new physics with their detector validation datasets. The validation of the detector response may be performed using a dedicated run with $\mu^+$, collecting data below the Michel edge, $E_e\lesssim 52$ MeV; an alternative strategy using $\pi^+\rightarrow e^+ \nu_e$ may also be considered. We focus primarily on a search for a monoenergetic $e^+$ produced via two-body decays $\mu^+ \rightarrow e^+ X$ or $\pi^+\rightarrow e^+X$, with $X$ a light new physics particle. Mu2e can potentially explore new parameter space beyond present astrophysical and laboratory constraints for a set of well motivated models including: axion like particles with flavor violating couplings ($\mu^+ \rightarrow e^+ a$), massive $Z'$ bosons ($\mu^+ \rightarrow Z' e^+$), and heavy neutral leptons ($\pi^+\rightarrow e^+N$). The projected sensitivities presented herein can be achieved in a matter of days.

==> Commands/flags.tex <==
\newcommand{\jure}[1]{\textcolor{red}{[{\bf JZ}: #1]}}
\newcommand{\ryan}[1]{\textcolor{blue}{[{\bf RP}: #1]}}
\newcommand{\richard}[1]{\textcolor{Brown}{[{\bf RH}: #1]}}

==> Commands/ryansCommands.tex <==
\newcommand{\citer}[1]{Ref. \cite{#1}}
\def\iu{\mathrm{i}}
\def\e{\mathrm{e}}
\def\Ldet{\ell}
\def\Ldec{\lambda}
